The Impact of Mobility between Rural Areas and Forests on the Spread of Zika

A mathematical model of Zika virus transmission incorporating human movement between rural areas and nearby forests is presented to investigate the role of human movement in the spread of Zika virus infections in human and mosquito populations. Proportions of both susceptible and infected humans living in rural areas are assumed to move to nearby forest areas. Direct, indirect and vertical transmission routes are incorporated for all populations. Mathematical analysis of the proposed model has been presented. The analysis starts with normalizing the proposed model. Positivity and boundedness of solutions to the normalized model have been then addressed. The basic reproduction number has been calculated using the next generation matrix method and its relation to the three routes of disease transmission has been presented. The sensitivity analysis of the basic reproduction number to all model parameters has been investigated. The analysis also includes existence and stability of disease free and endemic equilibrium points. Bifurcation analysis has been also carried out. Finally, numerical solutions to the normalized model have been obtained to confirm the theoretical results and to demonstrate the impact of human movement in the disease transmission in human and mosquito populations.

==> Mybib.tex <==
@article{ngm,
  title={Reproduction numbers and sub-threshold endemic equilibria for compartmental models of disease transmission},
  author={Van den Driessche, P. and Watmough, J.},
  journal={Mathematical biosciences},
  volume={180},
  number={1-2},
  pages={29--48},
  year={2002},
  publisher={Elsevier},
  doi = {10.1016/S0025-5564(02)00108-6}
}


@article{gas,
  title={On the computation of R0 and its role on global stability},
  author={Castilla-Chavez, C. and Feng, Z. and Huang, W.},
  journal={Biometrics},
  volume={125},
   pages={31-65},
  year={2001},
  doi= {10.1007/978-1-4757-3667-0_13}
}

@inproceedings{routh,
  title={Routh stability array method based reduced model of single machine infinite bus with power system stabilizer},
  author={Sambariya, D.K. and Prasad, R.},
  booktitle={International Conference on Emerging Trends in Electrical, Communication and Information Technologies (ICECIT-2012)},
  pages={27--34},
  year={2012},
  doi={10.13140/RG.2.1.4041.8325}
}

@article{dsr,
  title={Recent extentions of Descartes' rule of signs},
  author={Curtiss, D.R.},
  journal={Annals of Mathematics},
  pages={251--278},
  year={1918},
  publisher={JSTOR},
  doi={10.2307/1967494}
}

@book{soto,
  title={Differential equations: a dynamical systems approach: higher-dimensional systems},
  author={Hubbard, J. H and West, B. H.},
  volume={18},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@inproceedings{nsens,
  title={Sensitivity analysis in a dengue epidemiological model},
  author={Rodrigues, H. S. and Monteiro, M. T. T. and Torres, D. FM},
  booktitle={Conference Papers in Science},
  volume={2013},
  year={2013},
  organization={Hindawi},
  doi={10.1155/2013/721406}
}

@article{sens,
  title={Reproduction numbers of infectious disease models},
  author={Van den Driessche, P.},
  journal={Infectious Disease Modelling},
  volume={2},
  number={3},
  pages={288--303},
  year={2017},
  publisher={Elsevier},
  doi={10.1016/j.idm.2017.06.002}




@article{biting,
  title={Zika virus dynamics: When does sexual transmission matter?},
  author={Maxian, O. and Neufeld, A. and Talis, E. J. and Childs, L. M. and Blackwood, J. C.},
  journal={Epidemics},
  volume={21},
  pages={48--55},
  year={2017},
  publisher={Elsevier},
  doi = {10.1016/j.epidem.2017.06.003}
}

@article{vdeath,
  title={Mathematical modeling of Zika virus},
  author={Bonyah, E. and Okosun, K. O.},
  journal={Asian Pacific Journal of Tropical Disease},
  volume={6},
  number={9},
  pages={673--679},
  year={2016},
  publisher={Elsevier},
 doi={10.1016/S2222-1808(16)61108-8}
}

@article{gamma,
  title={A mathematical model for Zika virus transmission dynamics with a time-dependent mosquito biting rate},
  author={Suparit, P. and Wiratsudakul, A. and Modchang, C.},
  journal={Theoretical Biology and Medical Modelling},
  volume={15},
  number={1},
  pages={11},
  year={2018},
  publisher={Springer},
  doi={10.1186/s12976-018-0083-z}
}

@article{6,
  title={Guillain-Barr{\'e} Syndrome outbreak associated with Zika virus infection in French Polynesia: a case-control study},
  author={Cao-Lormeau, V-M.and Blake, A. and Mons, S. and Last{\`e}re, S. and Roche, C. and Vanhomwegen, J. and Dub, T.and Baudouin, L. and Teissier, A. and Larre, P. and others},
  journal={The Lancet},
  volume={387},
  number={10027},
  pages={1531--1539},
  year={2016},
  publisher={Elsevier},
  doi={10.1016/S0140-6736(16)00562-6}
}

@inproceedings{*,
  title={Mathematical modeling of Zika virus disease with nonlinear incidence and optimal control},
  author={Goswami, N. K. and Srivastav, A. K. and Ghosh, M. and Shanmukha, B.},
  booktitle={Journal of Physics: Conference Series},
  volume={1000},
  pages={1-16},
  year={2018},
  doi={10.1088/1742-6596/1000/1/012114}
}

@article{****,
  title={Mathematical model of zika virus dynamics with vector control and sensitivity analysis},
  author={Biswas, S. K. and Ghosh, U. and Sarkar, S.},
  journal={Infectious Disease Modelling},
  volume={5},
  pages={23--41},
  year={2020},
  publisher={Elsevier},
  doi={10.1016/j.idm.2019.12.001}
}

@article{19,
  title={Zika threatens to become a huge worldwide pandemic},
  author={Troncoso, A.},
  journal={Asian Pacific Journal of Tropical Biomedicine},
  volume={6},
  number={6},
  pages={520--527},
  year={2016},
  publisher={Elsevier},
  doi={10.1016/j.apjtb.2016.04.004}
}

@article{5,
  title={Possible association between Zika virus infection and microcephaly—Brazil},
  author={Schuler-Faccini, L. and Ribeiro, E. M. and Feitosa, I. ML and Horovitz, D. DG and Cavalcanti, D. P. and Pessoa, A. and Doriqui, M. J. R. and Neri, J. I. and de Pina Neto, J. M. and Wanderley, H. YC and others},
  journal={Morbidity and Mortality Weekly Report},
  volume={65},
  number={3},
  pages={59--62},
  year={2016},
  publisher={JSTOR},
  doi={10.15585/mmwr.mm6503e2}
}

@article{7,
  title={Zika virus infection, Cambodia, 2010},
  author={Heang, V. and Yasuda, C. Y. and Sovann, L. and Haddow, A. D. and da Rosa, A. P. T. and Tesh, R. B. and Kasper, M. R.},
  journal={Emerging infectious diseases},
  volume={18},
  number={2},
  pages={349},
  year={2012},
  publisher={Centers for Disease Control and Prevention},
  doi={10.3201/eid1802.111224}
}
@article{**,
  title={A theoretical model for Zika virus transmission},
  author={Bonyah, E. and Khan, M. A. and Okosun, KO and Islam, S.},
  journal={PloS one},
  volume={12},
  number={10},
  pages={e0185540},
  year={2017},
  publisher={Public Library of Science San Francisco, CA USA},
  doi={10.1371/journal.pone.0185540}
}

@article{***,
  title={Mathematical model of Zika virus with vertical transmission},
  author={Agusto, F. B. and Bewick, S. and Fagan, W. F.},
  journal={Infectious Disease Modelling},
  volume={2},
  number={2},
  pages={244--267},
  year={2017},
  publisher={Elsevier},
  doi={10.1016/j.idm.2017.05.003}
}

@article{4,
  title={Zika virus outbreak, bahia, brazil},
  author={Campos, G. S. and Bandeira, A. C. and Sardi, S. I.},
  journal={Emerging infectious diseases},
  volume={21},
  number={10},
  pages={1885},
  year={2015},
  publisher={Centers for Disease Control and Prevention},
  doi={10.3201/eid2110.150847}
}

@article{song,
  title={Dynamical models of tuberculosis and their applications},
  author={Castillo-Chavez, C. and Song, B.},
  journal={Mathematical Biosciences \& Engineering},
  volume={1},
  number={2},
  pages={361},
  year={2004},
  publisher={American Institute of Mathematical Sciences},
  doi={10.3934/mbe.2004.1.361}
}

@article{livelihoods,
  title={Interaction between rural people’s basic needs and forest products: A case study of the Katha District of Myanmar},
  author={Hlaing, Z. C. and Kamiyama, C. and Saito, O.},
  journal={International Journal of Forestry Research},
  volume={2017},
  year={2017},
  publisher={Hindawi},
  doi={10.1155/2017/2105012}
}

@article{matcont,
  title={New features of the software MatCont for bifurcation analysis of dynamical systems},
  author={Dhooge, A. and Govaerts, W. and Kuznetsov, Y. A. and Meijer, H. G. E. and Sautois, B.},
  journal={Mathematical and Computer Modelling of Dynamical Systems},
  volume={14},
  number={2},
  pages={147--175},
  year={2008},
  publisher={Taylor \& Francis},
  doi={10.1080/13873950701742754}
}

@article{Bueno,
  title={Animals in the Zika virus life cycle: what to expect from megadiverse Latin American countries},
  author={Bueno, M. G. and Martinez, N. and Abdalla, L. and Duarte dos Santos, C.  N. and Chame, M.},
  journal={PLoS neglected tropical diseases},
  volume={10},
  number={12},
  pages={e0005073},
  year={2016},
  publisher={Public Library of Science San Francisco, CA USA},
  doi={10.1371/journal.pntd.0005073}
}

@article{Dudley,
  title={A rhesus macaque model of Asian-lineage Zika virus infection},
  author={Dudley, D. M. and Aliota, M. T. and Mohr, E.L. and Weiler, A. M. and Lehrer-Brey, G. and Weisgrau, K. L. and Mohns, M. S. and Breitbach, Me. E. and Rasheed, M. N. and Newman, C. M. and others},
  journal={Nature communications},
  volume={7},
  number={1},
  pages={1-9},
  year={2016},
  publisher={Nature Publishing Group},
  doi={10.1101/046334}
  }

@article{MMWR,
  title={Interim Guidelines for Pregnant Women During a Zika Virus Outbreak—United States, 2016},
  author={Petersen, E. E. and Staples, J. E. and Meaney-Delman, D. and Fischer, M.and Ellington, S. R and Callaghan, W. M and Jamieson, D. J}, 
   volume={65},
  pages={30–33},
  year={2016},
  doi={10.15585/mmwr.mm6502e1}
}

@article{Than,
  title={Vertical transmission of Zika virus in Aedes aegypti mosquitoes},
  author={Thangamani, S. and Huang, J. and Hart, C. E. and Guzman, H. and Tesh, R. B.},
  journal={The American journal of tropical medicine and hygiene},
  volume={95},
  number={5},
  pages={1169-1173},
  year={2016},
  publisher={ASTMH},
  doi={10.1371/journal.pntd.0008776}
}

@article{CDC1,
title = {Zika: Transmission and Risks},
author = {CDC},
journal = {https://www.cdc.gov/zika/transmission/}
}


@article{brasil2020zika,
  title={Zika virus vertical transmission in children with confirmed antenatal exposure},
  author={Brasil, P. and Vasconcelos, Z. and Kerin, T. and Gabaglia, C. R. and Ribeiro, I. P. and Bonaldo, M. C. and Damasceno, L. and Pone, M. V. and Pone, S. and Zin, A. and others},
  journal={Nature communications},
  volume={11},
  number={1},
  pages={1--8},
  year={2020},
  publisher={Nature Publishing Group},
  doi={ 10.1038/s41467-020-17331-0}
}

@article{lai2020vertical,
  title={Vertical transmission of zika virus in Aedes albopictus},
  author={Lai, Z. and Zhou, T. and Zhou, J. and Liu, S. and Xu, Y. and Gu, J. and Yan, G. and Chen, X.-G.},
  journal={PLoS neglected tropical diseases},
  volume={14},
  number={10},
  pages={e0008776},
  year={2020},
  publisher={Public Library of Science San Francisco, CA USA},
  doi={10.1371/journal.pntd.0008776}
}






